OMEGA: Efficient Occlusion-Aware Navigation for Air-Ground Robot in Dynamic Environments via State Space Model

Air-ground robots (AGRs) are widely used in surveillance and disaster response due to their exceptional mobility and versatility (i.e., flying and driving). Current AGR navigation systems perform well in static occlusion-prone environments (e.g., indoors) by using 3D semantic occupancy networks to predict occlusions for complete local mapping and then computing Euclidean Signed Distance Field (ESDF) for path planning. However, these systems face challenges in dynamic, severe occlusion scenes (e.g., crowds) due to limitations in perception networks' low prediction accuracy and path planners' high computation overhead. In this paper, we propose OMEGA, which contains OccMamba with an Efficient AGR-Planner to address the above-mentioned problems. OccMamba adopts a novel architecture that separates semantic and occupancy prediction into independent branches, incorporating two mamba blocks within these branches. These blocks efficiently extract semantic and geometric features in 3D environments with linear complexity, ensuring that the network can learn long-distance dependencies to improve prediction accuracy. Semantic and geometric features are combined within the Bird's Eye View (BEV) space to minimise computational overhead during feature fusion. The resulting semantic occupancy map is then seamlessly integrated into the local map, providing occlusion awareness of the dynamic environment. Our AGR-Planner utilizes this local map and employs kinodynamic A* search and gradient-based trajectory optimization to guarantee planning is ESDF-free and energy-efficient. Extensive experiments demonstrate that OccMamba outperforms the state-of-the-art 3D semantic occupancy network with 25.0% mIoU. End-to-end navigation experiments in dynamic scenes verify OMEGA's efficiency, achieving a 96% average planning success rate. Code and video are available at https://jmwang0117.github.io/OMEGA/.

==> sup.tex <==
\section{Appendix}
\subsection{Details}
\subsubsection{The Voxel Interaction of LiDAR and Camera}
Fig.~\ref{fig:suppl_feat} (a) illustrates the challenge of aligning images and point clouds caused by inaccurate extrinsic parameters. Direct geometric alignment is difficult to achieve. To address the accumulation of errors resulting from misalignment, we propose GSFusion. This method searches for nearby features to ensure both geometric and semantic alignment, enabling each LiDAR voxel feature to interact with K neighboring lifted pixel features in the fusion process. This expands the perception field, allowing for a more comprehensive and robust fusion of image and point features.
Furthermore, Fig.~\ref{fig:suppl_feat} (b) highlights the impact of the sparsity of LiDAR point clouds on voxel interaction with the camera. To address this, the rendering process ensures dense representations for LiDAR features, camera features, or LiDAR-camera features, as depicted in Fig.~\ref{fig:suppl_feat} (c). This ensures sufficient voxel interaction and improves overall performance.
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{fig/suppl_feat.pdf}
    \caption{(a) illustrates the inaccurate calibrations between the projected points and the corresponding images.
(b) displays the sparse distribution of projected LiDAR points.
(c) showcases the rendered depth obtained from the fusion of LiDAR-camera features.}
    \label{fig:suppl_feat}
\end{figure}

\begin{table*}[t]
\setlength{\tabcolsep}{0.0045\linewidth}
\newcommand{\classfreq}[1]{{~\tiny(\semkitfreq{#1}\%)}}  %
\centering
\caption{\textbf{3D Semantic occupancy prediction results on nuScenes-Occupancy validation set.} We report the geometric metric IoU, semantic metric mIoU, and the IoU for each semantic class. The C, D, and L denotes camera, depth, and LiDAR, respectively. \textbf{Bold} represents the best score.}
\resizebox{.85\linewidth}{!}{
\begin{tabular}{l|c | c c | c c c c c c c c c c c c c c c c}
    \toprule
    Method
    & \makecell[c]{Modality}
    & IoU& mIoU
    & \rotatebox{90}{\textcolor{nbarrier}{$\blacksquare$} barrier}
    & \rotatebox{90}{\textcolor{nbicycle}{$\blacksquare$} bicycle}
    & \rotatebox{90}{\textcolor{nbus}{$\blacksquare$} bus}
    & \rotatebox{90}{\textcolor{ncar}{$\blacksquare$} car}
    & \rotatebox{90}{\textcolor{nconstruct}{$\blacksquare$} const. veh.}
    & \rotatebox{90}{\textcolor{nmotor}{$\blacksquare$} motorcycle}
    & \rotatebox{90}{\textcolor{npedestrian}{$\blacksquare$} pedestrian}
    & \rotatebox{90}{\textcolor{ntraffic}{$\blacksquare$} traffic cone}
    & \rotatebox{90}{\textcolor{ntrailer}{$\blacksquare$} trailer}
    & \rotatebox{90}{\textcolor{ntruck}{$\blacksquare$} truck}
    & \rotatebox{90}{\textcolor{ndriveable}{$\blacksquare$} drive. suf.}
    & \rotatebox{90}{\textcolor{nother}{$\blacksquare$} other flat}
    & \rotatebox{90}{\textcolor{nsidewalk}{$\blacksquare$} sidewalk}
    & \rotatebox{90}{\textcolor{nterrain}{$\blacksquare$} terrain}
    & \rotatebox{90}{\textcolor{nmanmade}{$\blacksquare$} manmade}
    & \rotatebox{90}{\textcolor{nvegetation}{$\blacksquare$} vegetation} \\
    % & mIoU\\
    \midrule
    MonoScene~\cite{cao2022monoscene} & C   & 18.4 & 6.9 & 7.1  & 3.9  &  9.3 &  7.2 & 5.6  & 3.0  &  5.9& 4.4& 4.9 & 4.2 & 14.9 & 6.3  & 7.9 & 7.4  & 10.0 & 7.6 \\
  
    TPVFormer~\cite{huang2023tri} &C &  15.3 &  7.8 & 9.3  & 4.1  &  11.3 &  10.1 & 5.2  & 4.3  & 5.9 & 5.3&  6.8& 6.5 & 13.6 & 9.0  & 8.3 & 8.0  & 9.2 & 8.2 \\

        3DSketch~\cite{chen20203d} &  C\&D & 25.6 & 10.7  & 12.0 &  5.1 &  10.7 &  12.4 & 6.5  & 4.0  & 5.0 & 6.3&  8.0&  7.2& 21.8 &  14.8 & 13.0 &  11.8 & 12.0 & 21.2 \\
        
        AICNet~\cite{li2020anisotropic} & C\&D   &   23.8 & 10.6  & 11.5  & 4.0  & 11.8  & 12.3&  5.1 & 3.8  & 6.2  & 6.0 & 8.2&  7.5&  24.1 & 13.0 & 12.8  & 11.5 & 11.6  &  20.2\\

        LMSCNet~\cite{roldao2020lmscnet} & L &   27.3 & 11.5 & 12.4&  4.2 & 12.8  & 12.1  & 6.2  &  4.7 & 6.2 & 6.3&  8.8&  7.2& 24.2 & 12.3  & 16.6 & 14.1  & 13.9 & 22.2 \\

        
    JS3C-Net~\cite{yan2021sparse} &L &   30.2  & 12.5 & 14.2 & 3.4  & 13.6  & 12.0  & 7.2  &  4.3 & 7.3 & 6.8&  9.2& 9.1 & 27.9 & 15.3  & 14.9 & 16.2  & 14.0 & 24.9 \\
    
        M-CONet~\cite{wang2023openoccupancy} & C\&L &   29.5 & 20.1 &  23.3  & 13.3& 21.2 & 24.3& \textbf{15.3}  & 15.9& 18.0 & 13.3 & 15.3 & 20.7 & 33.2 & 21.0 & 22.5  & 21.5 &19.6 & 23.2  \\ \midrule
        Co-Occ (Ours) & C\&L &\textbf{30.6}&\textbf{21.9}&\textbf{26.5}  &\textbf{16.8}&\textbf{22.3}&\textbf{27.0}&10.1&\textbf{20.9}&\textbf{20.7} &\textbf{14.5 }&\textbf{16.4} &\textbf{21.6}&\textbf{36.9}&\textbf{23.5}&\textbf{25.5} &\textbf{23.7} &\textbf{20.5} &\textbf{23.5} \\
    \bottomrule

\end{tabular}}

\label{tab:suppl_nusc}
\end{table*}

\begin{figure*}[h]
    \centering
    \includegraphics[width=\linewidth]{fig/suppl_nusc.pdf}
    \caption{The additional qualitative comparisons results on nuScenes validation set~\cite{behley2019semantickitti}. The leftmost column shows the input surrounding images and LiDAR sweeps, the following three columns visualize the 3D semantic occupancy prediction from SurroundOcc~\cite{wei2023surroundocc} (SurroundOcc predicts results using only cameras), M-CONet~\cite{wang2023openoccupancy}, our Co-Occ, and the annotation from~\cite{wei2023surroundocc}. \textbf{Better viewed when zoomed in.}}
    \label{fig:suppl_nusc}
\end{figure*}

\begin{figure*}[h]
    \centering
    \includegraphics[width=\linewidth]{fig/suppl_kitti.pdf}
    \caption{The additional qualitative comparisons results on SemanticKITTI validation set. The input monocular image and LiDAR sweeps are shown on the left and the 3D semantic occupancy results from OccFormer~\cite{zhang2023occformer} (OccFormer predicts results using only mono image), M-CONet~\cite{wang2023openoccupancy}, our Co-Occ, and the annotations are then visualized sequentially. \textbf{Better viewed when zoomed in.}}
    \label{fig:suppl_kitti}
\end{figure*}
\subsubsection{Other Implementation Details}
In our implicit volume rendering regularization, we employ two Multi-Layer Perceptron (MLP) networks as our density head and color head. These MLP networks are utilized to generate the density grid and color grid from the sampled frustum features. The color head consists of three layers of MLP, while the density head consists of either one layer of MLP or a Linear layer. This configuration strikes a balance between training memory requirements and rendering performance.
\subsection{Evaluation Metrics}
\noindent\textbf{IoU metrics.}
The Intersection over Union (IoU) is a metric used to determine whether a voxel is occupied or empty~\cite{caesar2020nuscenes, wang2023openoccupancy}. It treats all occupied voxels as the occupied class and all others as the empty class. The IoU is calculated as follows: 
\begin{equation} 
\rm{IoU} = \frac{TP_o}{TP_o+FP_o+FN_o}, 
\end{equation} 
where $TP_o, FP_o, FN_o$ represent the number of true positives, false positives, and false negatives of the occupied class, respectively.

\noindent\textbf{mIoU metrics.}
The mean Intersection over Union (mIoU) is a metric that calculates the average IoU for each semantic class. It is defined as follows:
\begin{equation}
    \rm{mIoU} = \frac{1}{N_c}\sum_{c=1}^{N_c}\frac{TP_c}{TP_c+FP_c+FN_c},
\end{equation}
where $TP_c, FP_c, FN_c$ represent the number of true positives, false positives, and false negatives for class $c$, respectively, and $N_c$ is the total number of classes.



\subsection{More Results}
\noindent\textbf{More Quantitative Results on NuScenes dataset.}
We supply the 3D semantic occupancy prediction results on different voxel resolutions. As the openoccupancy benchmark~\cite{wang2023openoccupancy}, the voxel resolution is $0.2m$ in a volume of $512\times512\times40$ for occupancy predictions. As presented in Tab.~\ref{tab:suppl_nusc}, we test other method on nuScenes-occupancy validation set~\cite{caesar2020nuscenes, wang2023openoccupancy}. our Co-Occ method obtain \textbf{1.8\%} mIoU improvement among the camera-LiDAR fusion-based M-CONet. Besides, the scores of most semantic classes have a large margin improvement. These experiments validate the effectiveness of our method that not only obatin better performance on one voxel resolution.




\noindent\textbf{More Visualization Results on NuScenes Dataset.}
Due to space constraints, we have included additional visual results in Fig. \ref{fig:suppl_nusc}. These results demonstrate that our method has more precise details compared to the camera-only method~\cite{wei2023surroundocc}, while also achieving greater consistency than other LiDAR-camera fusion-based methods~\cite{wang2023openoccupancy}. Furthermore, the effectiveness of our methods in challenging conditions is validated through the \textit{video demo}.


\noindent\textbf{More Visualization Results on SemanticKITTI Dataset.}
Similarly, we present additional qualitative results using the SemanticKITTI validation dataset in Fig.~\ref{fig:suppl_kitti}. Our method's semantic predictions clearly outperform not only in dynamic objects like cars but also in capturing the complementary aspects of road and vegetation. This showcases the effectiveness and versatility of our approach.


\noindent\textbf{Video Demo.}
To provide a comprehensive understanding of our method and showcase the dynamic performance of our results, we have prepared a video demo. This demo visually presents our continuous video visualization results, allowing you to observe our method in action and gain a deeper understanding of its process. 
